Point-SAM: Promptable 3D Segmentation Model for Point Clouds

The development of 2D foundation models for image segmentation has been significantly advanced by the Segment Anything Model (SAM). However, achieving similar success in 3D models remains a challenge due to issues such as non-unified data formats, poor model scalability, and the scarcity of labeled data with diverse masks. To this end, we propose a 3D promptable segmentation model Point-SAM, focusing on point clouds. We employ an efficient transformer-based architecture tailored for point clouds, extending SAM to the 3D domain. We then distill the rich knowledge from 2D SAM for Point-SAM training by introducing a data engine to generate part-level and object-level pseudo-labels at scale from 2D SAM. Our model outperforms state-of-the-art 3D segmentation models on several indoor and outdoor benchmarks and demonstrates a variety of applications, such as interactive 3D annotation and zero-shot 3D instance proposal. Codes and demo can be found at https://github.com/zyc00/Point-SAM.

==> tables/ablation-scannet-results.tex <==
\begin{table}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|ccccc}
\toprule
Dataset          & Method    & IoU@1 & IoU@3 & IoU@5 & IoU@7 & IoU@10 \\ \midrule
PartNet-Mobility & AGILE3D   & 26.4  & 40.8  & 50.8  & 57.4  & 61.9   \\
                 & Point-SAM & \textbf{33.5}  & \textbf{48.5}  & \textbf{57.0}  & \textbf{61.2}  & \textbf{66.8}   \\
                 & Point-SAM* & \textbf{47.9}  & \textbf{67.7}  & \textbf{74.2}  & \textbf{77.0}  & \textbf{78.6}   \\
                 \midrule
ScanObjNN        & AGILE3D   & \textbf{34.8}  & 52.0  & 61.6  & 67.2  & \textbf{72.3}   \\
                 & Point-SAM & 32.0  & \textbf{56.7}  & \textbf{63.2}  & \textbf{68.8}  & 70.5   \\
                 & Point-SAM* & \textbf{49.4}  & \textbf{75.3}  & \textbf{82.0}  & \textbf{84.8}  & \textbf{86.3}   \\
                 \midrule
S3DIS            & AGILE3D   & \textbf{58.7}  & \textbf{77.4}  & \textbf{83.6}  & \textbf{86.4}  & \textbf{88.5}   \\
                 & Point-SAM & 38.8  & 67.1  & 72.2  & 78.9  & 80.6   \\ 
                 & Point-SAM* & 47.6  & \textbf{78.4}  & \textbf{86.2}  & \textbf{89.2}  & \textbf{90.4}   \\
                 \midrule
KITTI360         & AGILE3D   & 34.8  & 42.7  & 44.4  & 45.8  & 49.6   \\
                 & Point-SAM & \textbf{44.0}  & \textbf{67.1}  & \textbf{72.2}  & \textbf{78.9}  & \textbf{80.8}   \\ 
                 & Point-SAM* & \textbf{49.4}  & \textbf{74.4}  & \textbf{87.1}  & \textbf{84.3}  & \textbf{85.8}   \\
                 \bottomrule
\end{tabular}
}
\centering
\caption{Quantitative results for Point-SAM trained on ScanNet. For the equitable comparison with AGILE3D, we train Point-SAM* on ScanNet following the setting of AGILE3D. Then we show the IoU results under the same setting of Table 3. in the paper. Our final version model is also listed as Point-SAM.}
\end{table}

==> tables/ablation_scannet.tex <==
\begin{table}[ht]{}
\centering
\caption{Quantitative results for Point-SAM trained on ScanNet. Point-SAM* is trained on ScanNet following the setting of AGILE3D. Point-SAM is our original setting}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cc|ccccc}
\toprule
Dataset          & Method    & IoU@1 & IoU@3 & IoU@5 & IoU@7 & IoU@10 \\ \midrule
PartNet-Mobility & AGILE3D   & 26.4  & 40.8  & 50.8  & 57.4  & 61.9   \\
                 & Point-SAM* & 33.5  & 48.5  & 57.0  & 61.2  & 66.8   \\
                 & Point-SAM & \textbf{47.9}  & \textbf{67.7}  & \textbf{74.2}  & \textbf{77.0}  & \textbf{78.6}   \\
                 \midrule
ScanObjNN        & AGILE3D   & 34.8  & 52.0  & 61.6  & 67.2  & 72.3   \\
                 & Point-SAM* & 32.0  & 56.7  & 63.2  & 68.8  & 70.5   \\
                 & Point-SAM & \textbf{49.4}  & \textbf{75.3}  & \textbf{82.0}  & \textbf{84.8}  & \textbf{86.3}   \\
                 \midrule
S3DIS            & AGILE3D   & \textbf{58.7}  & 77.4  & 83.6  & 86.4  & 88.5   \\
                 & Point-SAM* & 38.8  & 67.1  & 72.2  & 78.9  & 80.6   \\ 
                 & Point-SAM & 47.6  & \textbf{78.4}  & \textbf{86.2}  & \textbf{89.2}  & \textbf{90.4}   \\
                 \midrule
KITTI360         & AGILE3D   & 34.8  & 42.7  & 44.4  & 45.8  & 49.6   \\
                 & Point-SAM* & 44.0  & 67.1  & 72.2  & 78.9  & 80.8   \\ 
                 & Point-SAM & \textbf{49.4}  & \textbf{74.4}  & \textbf{87.1}  & \textbf{84.3}  & \textbf{85.8}   \\
                 \bottomrule
\end{tabular}
}
\label{tab:scannet}
\centering
\end{table}
